Sharp analysis of out-of-distribution error for "importance-weighted" estimators in the overparameterized regime

Overparameterized models that achieve zero training error are observed to generalize well on average, but degrade in performance when faced with data that is under-represented in the training sample. In this work, we study an overparameterized Gaussian mixture model imbued with a spurious feature, and sharply analyze the in-distribution and out-of-distribution test error of a cost-sensitive interpolating solution that incorporates "importance weights". Compared to recent work Wang et al. (2021), Behnia et al. (2022), our analysis is sharp with matching upper and lower bounds, and significantly weakens required assumptions on data dimensionality. Our error characterizations also apply to any choice of importance weights and unveil a novel tradeoff between worst-case robustness to distribution shift and average accuracy as a function of the importance weight magnitude.

==> experiment.tex <==
\section{Numerical results}\label{sec:exp_result}
%

==> note.tex <==
\section{Notes:}
% \begin{enumerate}
%     \item Next goal: show the error upper bound can be potentially improved by increasing $n_+$ only.
%     \item We study the isotropic covariance ($\bSigma=\I$) and ridge estimator.
% \end{enumerate}
% \paragraph{Experiment result}
% First of all, we show the result with data imbalance of $n_+:n_-=96:4$. Although the data imbalance is severe, we data imbalance ratio keeps the same as n increases. Hence, $n_-$ increases as $n$ increases.
% \begin{figure}[H]
% \centering 
%  \includegraphics[width=120mm]{figures/3_1.png}
%  \caption{Cost-sensitive MNI with different ridge estimator parameter $\tau$. The result shows that when $n$ increases and it's out of $d\geq Cn^2\log(n/\delta)$ regime, the worst group error starts increasing.}
% \end{figure}

% \begin{figure}[H]
% \centering 
%  \includegraphics[width=100mm]{figures/3_2.png}
%  \caption{MNI with different ridge estimator parameter $\tau$.}
% \end{figure}

% \begin{figure}[H]
% \centering 
%  \includegraphics[width=120mm]{figures/3_3.png}
%  \caption{cMNI and MNI with different ridge estimator parameter $\tau$. The result shows that in the $d\geq Cn^2\log(n/\delta)$ regime, cMNI improves the worst group error.}
% \end{figure}
% Next, we show the result for fixed $n_-=10$.

% \begin{figure}[H]
% \centering 
%  \includegraphics[width=120mm]{figures/4_1.png}
%  \caption{Cost-sensitive MNI with different ridge estimator parameter $\tau$. The result shows that when $n$ increases the worst group error goes up.}
% \end{figure}

% \begin{figure}[H]
% \centering 
%  \includegraphics[width=120mm]{figures/4_2.png}
%  \caption{MNI with different ridge estimator parameter $\tau$.}
% \end{figure}
% We can conclude several findings
% \begin{enumerate}
%     \item Regularization helps extend the regime of $d\geq Cn^2\log(n/\delta)$.
%     \item Regularization provides better worst group error. (This is implicit in the bounds.)
%     \item Increase $n_+$ only doesn't provide better worst group error.
% \end{enumerate}
% \paragraph{Ridge estimator upper bound for w/o spurious correlation data}
% \begin{gather*}
%     \Riskf[b]{\hw}\leq \expf{- C_1 \frac{ \pts{\pts{1-\frac{n}{\tau + d}}\nnorm[2]{\bmu}^2-C_2\nnorm[2]{\bmu}}^2}{C_3\text{max}\{1, \frac{n^2\nnorm[2]{\bmu}^2}{\pts{\tau + d}^2}\}d + C_4\nnorm[2]{\bmu}^2}}
% \end{gather*}
% When it's in $d\geq Cn^2\log(n/\delta)$ regime,
% \begin{gather*}
%     \Riskf[b]{\hw}\leq \expf{- C_1 \frac{ \pts{\nnorm[2]{\bmu}^2-C_2\nnorm[2]{\bmu}}^2}{C_3d + C_4\nnorm[2]{\bmu}^2}}
% \end{gather*}
% % \paragraph{Ridge estimator upper bound for spurious correlation data}
% % \begin{gather*}
% %     \Riskf[b]{\hw}\leq\expf{-C_1\frac{ \pts{\alpha_+ R_b^2n_+ + \alpha_-R_{-b}^2n_-}}{C_2nd + C_3R_+\pts{\alpha_+ n_+ + \alpha_-n_-}}}
% % \end{gather*}
% % \paragraph{Ridge estimator lower bound for spurious correlation data}
% % \begin{gather*}
% %     \Riskf[b]{\hw}\geq C_1 \expf{- C_2 \frac{ \pts{\alpha_+R_b^2n_+ + \alpha_-R_{-b}^2n_-}}{d}}
% % \end{gather*}

In order to prove bounds for Ridge estimator, we need the following new primitives.

\begin{definition}\label{def:new_primitives}
    Let $\bv_0\in\R^n$ as any vector with $\nnorm[2]{\bv_0}=1$, and for $i=1,2$, we define the following basic primitives:
    \begin{gather}
        \szzk \coloneqq \bv_0^\top\XXki\bv_0,\quad \szik \coloneqq \bv_0^\top\XXki\bv_i, \quad \hizk \coloneqq \bd_i^\top\XXki\bv_0 \nonumber,\nonumber
    \end{gather}
\end{definition}
And, we have the following primitive bounds
\begin{lemma}\label{lem:new_primitive_bounds}
    % For primitives we defined in Def.~\ref{def:primitives}, for some $C_1,C_2,C_3,C_4,C_5>1$ and $\hc_m \coloneqq \frac{C_m+1}{C_m}$ and $\dc_m \coloneqq \frac{C_m-1}{C_m}$, we have the following bounds.
    We have the following upper and lower bounds for the basic primitives (Def.~\ref{def:new_primitives}):
    \begin{gather*}
        \hc_1\frac{1}{d}\leq \szzk \leq \hc_1 \frac{1}{d}\\
        -\frac{C_2\sqrt{n}}{d} \leq \szik \leq \frac{C_2\sqrt{n}}{d}\\
        -\frac{C_3 \sqrt{n}\nui}{d}\leq \hizk \leq \frac{C_3 \sqrt{n}\nui}{d}
    \end{gather*}
    % In the above, we specifically have $\hc_m = \frac{C_m+ 1}{C_m}, \dc_m = \frac{C_m - 1}{C_m}$ and $C_m > 1$.
\end{lemma}
\begin{proof}
    We first show all bounds for order $k=0$.\\
    $\bullet\; \szzz = \bv_0^\top\XXzi\bv_0 = \bv_0^\top\QQi\bv_0$. Based on Lemma~\ref{lem:wishart_bound} with $t=\sqrt{2\log\pts{n/\delta}}$, we have with probability at least $1-\frac{\delta^2}{n^2}$,
    \begin{align*}
        \szzz & \leq \frac{\nvz^2}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}} \leq \frac{1}{d'(n)\pts{1-\frac{2}{\sqrt{C}n}}} = \frac{\frac{\sqrt{C}n}{\sqrt{C}n-2}}{d'(n)}  \leq \pts{\frac{C_1+1}{C_1}}\frac{1}{d},
    \end{align*}
    where the second inequality follows by Assumption~\ref{asm:dataset_gen}(D) such that $\frac{1}{Cn^2} \geq \frac{\log(n/\delta)}{d'(n)}$. Similarly, 
    \begin{align*}
        \szzz & \geq \frac{\nvz^2}{d'(n) + \sqrt{4\log\pts{n/\delta} \cdot d'(n)} + 4\log\pts{1/\delta}} \geq \frac{n}{d'(n)\pts{1+\frac{2}{\sqrt{C}n}+\frac{4}{Cn}}} \geq \pts{\frac{C_1-1}{C_1}}\frac{1}{d}.
        % \siiz & \leq \frac{\nvi^2}{\lbf[\text{min}]{\QQ}} \\
        % &\leq \frac{\nvi^2}{\pts{\sqrt{d} -\sqrt{n} - \sqrt{2\log\pts{n/\delta}}}^2} \leq \frac{C_1n}{d},\\
        % \siiz & \geq \frac{\nvi^2}{\lbf[\text{max}]{\QQ}}\\
        % &\geq \frac{n}{\pts{\sqrt{d} +\sqrt{n} + \sqrt{2\log\pts{n/\delta}}}^2} \geq \frac{n}{C_1d}.
    \end{align*}
    $\bullet\;\sziz = \bv_0^\top\XXzi\bv_i = \bv_0^\top\QQi\bv_i$ for $i=1,2$. Note that this is a ``cross-term" primitive. Hence, 
    \begin{align*}
        \sziz &\leq \nvz\nvi\nnorm[2]{\QQi} \leq \frac{C\sqrt{n}}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}} \leq \frac{C\sqrt{n}}{d}.\\
        % &\leq \frac{Cn\nui}{d'(n)\pts{1-\frac{2}{\sqrt{Cn^2}}}}
        %
        \sziz &\geq -\nvz\nvi\nnorm[2]{\QQi} \geq \frac{-C\sqrt{n}}{d}.
        % \sziz &\leq\frac{1}{4}\pts{\frac{n+1}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}} - \frac{n-1}{d'(n) + \sqrt{4\log\pts{n/\delta} \cdot d'(n)} + 4\log\pts{n/\delta}}}\\
        % &\leq \frac{n+1}{4d'(n)\pts{1-\frac{2}{\sqrt{Cn^2}}}} - \frac{n-1}{4d'(n)\pts{1+\frac{2}{\sqrt{Cn^2}}+\frac{4}{Cn^2}}}\\
        % &\leq \pts{\frac{C_2+1}{C_2}}\frac{n+1}{4d}-\pts{\frac{C_2-1}{C_2}}\frac{n-1}{4d}.\\
        % %
        % \sziz &\geq \frac{1}{4}\pts{\frac{n-1}{d'(n) + \sqrt{4\log\pts{n/\delta} \cdot d'(n)} + 4\log\pts{n/\delta}} - \frac{n+1}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}}}\\
        % &\geq \frac{n-1}{4d'(n)\pts{1+\frac{2}{\sqrt{Cn^2}} +\frac{4}{Cn^2}}} - \frac{n+1}{4d'(n)\pts{1-\frac{2}{\sqrt{Cn^2}}}}\\
        % &\geq \pts{\frac{C_2-1}{C_2}}\frac{n-1}{4d}-\pts{\frac{C_2+1}{C_2}}\frac{n+1}{4d}.
        % \sotz &\leq\frac{1}{4}\pts{\frac{4n_+}{\lbf[\text{min}]{\QQ}} - \frac{4n_-}{\lbf[\text{max}]{\QQ}}}\\
        % &\leq \frac{C_1n_+}{d}-\frac{n_-}{C_1d}.\\
        % %
        % \sotz &\geq \frac{1}{4}\pts{\frac{4n_+}{\lbf[\text{max}]{\QQ}} - \frac{4n_-}{\lbf[\text{min}]{\QQ}}}\\
        % &\geq \frac{n_+}{C_1d}-\frac{C_1n_-}{d}.
    \end{align*}
    $\bullet \; \hizz = \bd_i^\top\XXzi\bv_0 = \bd_i^\top\QQi\bv_0$, for $i=1,2$. Hence,
    \begin{align*}
        \hizz &\leq \ndi\nvz\nnorm[2]{\QQi} \leq \frac{C\sqrt{n}\nui}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}} \leq \frac{C_4\sqrt{n}\nui}{d}.\\
        % &\leq \frac{Cn\nui}{d'(n)\pts{1-\frac{2}{\sqrt{Cn^2}}}}
        %
        \hizz &\geq -\ndi\nvz\nnorm[2]{\QQi} \geq \frac{-C_4\sqrt{n}\nui}{d}.
        % &\geq \frac{-Cn\nui}{d'(n) - \sqrt{4\log\pts{n/\delta} \cdot d'(n)}}\\
        % &\geq \frac{-Cn\nui}{d'(n)\pts{1-\frac{2}{\sqrt{Cn^2}}}}
        % \hijz &\leq \ndi\nvj\nnorm[2]{\QQi}\\
        % &\leq \frac{Cn\nui}{\lbf[\text{min}]{\QQ}}
        % \leq \frac{C_4n\nui}{d}.\\
        % %
        % \hijz &\geq -\ndi\nvj\nnorm[2]{\QQi} \geq \frac{-C_4n\nui}{d}.
    \end{align*}
    Next, we assume that the bounds for order $k=k$ are true, and we show the bounds for order $k=k+1$. The key idea is that the higher order primitives are a constant fraction of the previous-order primitives.\\
    $\bullet \; \szzkpo$.
    \begin{align*}
        &\szzkpo = \bv_0^\top\XXkpoi\bv_0\\
        &=\bv_0^\top\XXki\bv_0 - \bv_0^\top\XXki\bL_{k+1}\A_{k+1}^{-1}\bR_{k+1}\XXki\bv_0\\
        &= \szzk - \mts{\nukpo\szkpok,~\hkpozk,~\szkpok} \times\frac{\text{adj}(\A_{k+1})}{\det(\A_{k+1})}\begin{bmatrix}
        \nukpo\szkpok \\
        \szkpok \\
        \hkpozk
        \end{bmatrix}\\
        &= \frac{\szzk \det(\A_{k+1}) - \ffs[\A_{k+1}]{\szkpok, \hkpozk, \szkpok, \hkpozk}}{\det(\A_{k+1})}.
    \end{align*}
    Thus, we can apply Lemma~\ref{lem:aux_f_func} to get 
    \begin{align*}
        \szzkpo &\leq \frac{1}{\det(\A_{k+1})}\Bigg(\frac{C_4+1}{C_4}\szzk + \nukpo^2\normo{\szkpok}\normo{\szkpok}\\
        &+ \pts{1+\frac{1}{C_1}}\pts{\normo{\szkpok}\normo{\hkpozk} + \normo{\hkpozk}\normo{\szkpok}} + \normo{\skkkmo}\normo{\hkpozk}\normo{\hkpozk}\Bigg)\\
        & \leq \frac{1}{\det(\A_{k+1})} \pts{\frac{C_5+1}{C_5}\frac{1}{d}} \leq \frac{C_6+1}{C_6}\frac{1}{d},
    \end{align*}
    where in the last inequality we apply lower bound of $\det(\A_{k+1})$ in Lemma~\ref{lem:aux_det_bound}. Similarly, 
    \begin{align*}
        \szzkpo &\geq \frac{1}{\det(\A_{k+1})}\Bigg(\frac{C_4-1}{C_4}\szzk- \Bigg(\nukpo^2\normo{\szkpok}\normo{\szkpok}\\
        &+ \pts{1+\frac{1}{C_2}}\pts{\normo{\szkpok}\normo{\hkpozk} + \normo{\hkpozk}\normo{\szkpok}} + \normo{\skkkmo}\normo{\hkpozk}\normo{\hkpozk}\Bigg)\Bigg)\\
        & \geq \frac{1}{\det(\A_{k+1})} \pts{\frac{C_5-1}{C_5}\frac{1}{d}} = \frac{C_5-1}{C_5}\frac{1}{d}.
    \end{align*}
    $\bullet \; \szikpo$ for $i=1,2$.
    \begin{align*}
        \szikpo &= \bv_0^\top\XXkpoi\bv_i\\
        &=\bv_0^\top\XXki\bv_i - \bv_0^\top\XXki\bL_{k+1}\A_{k+1}^{-1}\bR_{k+1}\XXki\bv_i\\
        &= \szik - \mts{\nukpo\szkpok,~\hkpozk,~\szkpok} \times\frac{\text{adj}(\A_{k+1})}{\det(\A_{k+1})}\begin{bmatrix}
        \nukpo\sikpok \\
        \sikpok \\
        \hkpoik
        \end{bmatrix}\\
        &= \frac{\sotk \det(\A_{k+1}) - \ffs[\A_{k+1}]{\szkpok, \hkpozk, \sikpok, \hkpoik}}{\det(\A_{k+1})}.
    \end{align*}
    Thus, we can apply Lemma~\ref{lem:aux_f_func} to get 
    \begin{align*}
        \szikpo &\leq \frac{1}{\det(\A_{k+1})}\Bigg(\det(\A_{k+1})\szik + \nukpo^2\normo{\szkpok}\normo{\sikpok} + \normo{\skpokpok}\normo{\hkpozk}\normo{\hkpoik}\\
        &\myquad[2] + \pts{1+\frac{1}{C_1}}\pts{\normo{\szkpok}\normo{\hkpoik} + \normo{\hkpozk}\normo{\sikpok}}\Bigg)\\
        & \leq \frac{1}{\det(\A_{k+1})} \Bigg(\frac{C_2+1}{C_2}\frac{C_3\sqrt{n}}{d} + \frac{C_4+1}{C_4}\frac{C_5\sqrt{n}}{d}\frac{\nukpo^2 n}{d}+ \frac{C_6+1}{C_6}\frac{\nukpo^2n^2\sqrt{n}}{d^3}\\
        &+ \frac{C_7+1}{C_7}\Bigg(\frac{C_8\sqrt{n}}{d}\frac{\nukpo n}{d} + \frac{C_9+1}{C_9}\frac{\nukpo n\sqrt{n}}{d^2}\Bigg)\Bigg)\\
        & \leq \frac{C_{10}\sqrt{n}}{d},
    \end{align*}
    %
    where in the second inequality we apply lower bound of $\det(\A_{k+1})$ in Lemma~\ref{lem:aux_det_bound} and primitive bounds in order $k$, and in the last inequality, we apply Assumption~\ref{asm:dataset_gen}(C) such that $d \geq CR_+n$.  Similarly,
    \begin{align*}
        \szikpo &\geq \frac{1}{\det(\A_{k+1})}\Bigg(-\det(\A_{k+1})\szik -\Bigg(\nukpo^2\normo{\szkpok}\normo{\sikpok} + \normo{\skpokpok}\normo{\hkpozk}\normo{\hkpoik}\\
        &\myquad[2]+ \pts{1+\frac{1}{C_1}}\pts{\normo{\szkpok}\normo{\hkpoik} + \normo{\hkpozk}\normo{\sikpok}}\Bigg)\Bigg)\\
        & \geq \frac{1}{\det(\A_{k+1})} \Bigg(-\frac{C_2-1}{C_2}\frac{C_3\sqrt{n}}{d} - \frac{C_4+1}{C_4}\frac{C_5\sqrt{n}}{d}\frac{\nukpo^2 n}{d} - \frac{C_6+1}{C_6}\frac{\nukpo^2n^2\sqrt{n}}{d^3}\\
        &\myquad[1]  - \frac{C_7+1}{C_7}\Bigg(\frac{C_8\sqrt{n}}{d}\frac{\nukpo n}{d} + \frac{C_9+1}{C_9}\frac{\nukpo n\sqrt{n}}{d^2}\Bigg)\Bigg)\\
        & \geq -\frac{C_{10}\sqrt{n}}{d}.
    \end{align*}
    $\bullet \; \hizkpo = \bd_i^\top\XXkpoi\bv_0$, for $i=1,2$.
    \begin{align*}
        \hizkpo &= \bd_i^\top\XXkpoi\bv_0\\
        &=\bd_i^\top\XXki\bv_0 - \bd_i^\top\XXki\bL_{k+1}\A_{k+1}^{-1}\bR_{k+1}\XXki\bv_0\\
        &= \hizk - \mts{\nukpo\hikpok,~\tikpok,~\hikpok} \times\frac{\text{adj}(\A_{k+1})}{\det(\A_{k+1})}\begin{bmatrix}
        \nukpo\szkpok \\
        \szkpok \\
        \hkpozk
        \end{bmatrix}\\
        &= \frac{\hijk \det(\A_{k+1}) - \ffs[\A_{k+1}]{\hikpok, \tikpok, \szkpok, \hkpozk}}{\det(\A_{k+1})}.
    \end{align*}
    Thus, we can apply Lemma~\ref{lem:aux_f_func} to get 
    \begin{align*}
        \hizkpo &\leq \frac{1}{\det(\A_{k+1})}\Bigg(\det(\A_{k+1})\hizk + \nukpo^2\normo{\hikpok}\normo{\szkpok} + \normo{\skpokpok}\normo{\tikpok}\normo{\hkpozk}\\
        &\myquad[2] + \pts{1+\frac{1}{C_1}}\pts{\normo{\hikpok}\normo{\hkpozk} + \normo{\tikpok}\normo{\szkpok}}\Bigg)\\
        & \leq \frac{1}{\det(\A_{k+1})} \Bigg(\frac{C_2+1}{C_2}\frac{C_3\sqrt{n}\nui}{d} + \frac{C_4\nukpo^2\nui n\sqrt{n}}{d^2}\\
        &\myquad[2] + \frac{C_5+1}{C_5}\frac{\nui\nukpo^2n^2\sqrt{n}}{d^3} + \frac{C_6+1}{C_6}\frac{\nui\nukpo n\sqrt{n}}{d^2}\Bigg)\\
        & \leq \frac{C_7\sqrt{n}\nui}{d},
    \end{align*}
    %
    where in the second inequality we apply lower bound of $\det(\A_{k+1})$ in Lemma~\ref{lem:aux_det_bound} and primitive bounds in order $k$, and in the last inequality, we apply Assumption~\ref{asm:dataset_gen}(C) such that $d \geq CR_+n$. Similarly, 
    \begin{align*}
        \hizkpo &\geq \frac{1}{\det(\A_{k+1})}\Bigg(\det(\A_{k+1})\hizk -\Bigg( \nukpo^2\normo{\hikpok}\normo{\szkpok} + \normo{\skpokpok}\normo{\tikpok}\normo{\hkpozk}\\
        &\myquad[2] + \pts{1+\frac{1}{C_1}}\pts{\normo{\hikpok}\normo{\hkpozk} + \normo{\tikpok}\normo{\szkpok}}\Bigg)\Bigg)\\
        & \geq \frac{1}{\det(\A_{k+1})} \Bigg(-\frac{C_2+1}{C_2}\frac{C_3\sqrt{n}\nui}{d} - \frac{C_4\nukpo^2\nui n\sqrt{n}}{d^2}\\
        & \myquad[2]- \frac{C_5+1}{C_5}\frac{\nui\nukpo^2n^2\sqrt{n}}{d^3} - \frac{C_6+1}{C_6}\frac{\nui\nukpo n\sqrt{n}}{d^2}\Bigg)\\
        & \geq -\frac{C_7\sqrt{n}\nui}{d}.
    \end{align*}
\end{proof}


\begin{proposition}\label{pro:ridge_wst_upper_bound}
Under Assumption~\ref{asm:dataset_gen}, the generalization error of ridge estimator for each group $b \in \{+1,-1\}$ is upper bounded as
    \begin{gather}
        \Riskf[b]{\hw}\leq \expf{-C_1\frac{ \pts{\alpha_+ R_b^2n_+ + \alpha_-R_{-b}^2n_-}}{C_2d}}
    \end{gather}
    where $\alpha_\pm \coloneqq \frac{n_\pm/\Delta_\pm^2}{\nddpndd}=\frac{n_\pm/\Delta_\pm^2}{\nd}$ and $0 < \alpha_\pm < 1$.
\end{proposition}
\begin{proof}
    \begin{align}
        \frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} &= \frac{\pts{\y^\top\bDelta^{-1}\XXtaui\X\bmu_{+1}}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\nonumber\\
        &= \frac{\pts{\nut^2\stdtt + \nuo^2\stdot + \httdt + \hotdt}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\label{eq:ridge_maj_target_term},
    \end{align}
    where we reuse the primitives in Eq.~\eqref{eq:maj_target_primitive}. Next, we focus on upper bound the denominator.
    \begin{align*}
        &\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y\\
        &\leq \lambda_{\text{max}}\pts{\XX}\nnorm[2]{\XXtaui\bDelta^{-1}\y}^2\\
        &\leq \lambda_{\text{max}}\pts{\XX}\nnorm[2]{\XXtaui}^2\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \lambda_{\text{max}}\pts{\XX}\lambda_{\text{max}}\pts{\XXtaui}^2\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \frac{\lambda_{\text{max}}\pts{\XX}}{\lambda_{\text{min}}\pts{\XXtau}^2}\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \frac{\lambda_{\text{max}}\pts{\XX}}{\pts{\lambda_{\text{min}}\pts{\XX} + \tau}^2}\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \frac{\frac{1}{\lambda_{\text{min}}\pts{\XXi}}}{\pts{\frac{1}{\lambda_{\text{max}}\pts{\XXi}} + \tau}^2}\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \frac{\frac{1}{\umin{\nnorm[2]{\bv}=1}\;\bv^\top\XX\bv}}{\pts{\frac{1}{\umax{\nnorm[2]{\bv}=1}\;\bv^\top\XX\bv} + \tau}^2}\nnorm[2]{\bDelta^{-1}\y}^2\\
        &\leq \frac{C_1 d \nd}{\pts{d+\tau}^2},
    \end{align*}
    where the first two inequalities follow the property of spectral norm, and the last inequality follows by Lemma~\ref{lem:new_primitive_bounds} and $\nnorm[2]{\bDelta^{-1}\y}^2 = \nd$
    Plug this in Eq.~\eqref{eq:ridge_maj_target_term}, we have
    \begin{align*}
         \frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} &= \frac{\pts{\nut^2\stdtt + \nuo^2\stdot + \httdt + \hotdt}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\\
         &\geq \dfrac{\pts{\nut^2 \frac{\pts{\hc_1+\frac{1}{C_2}} \pts{\ndpnd}}{d+\tau} + \nuo^2 \frac{\hc_1 \pts{\ndmnd} + \frac{1}{C_2}\pts{\ndpnd}}{d+\tau}+\frac{C_3 \sqrt{n\nd}\nut}{d+\tau}+\frac{C_3 \sqrt{n\nd}\nuo}{d+\tau}}^2}{\frac{C_4\nd d}{\pts{d+\tau}^2}}\nonumber\\
         &\leq \dfrac{\pts{\splitdfrac{\nut^2 \pts{\hc_1+\frac{1}{C_2}} \pts{\ndpnd} + \nuo^2 \pts{\hc_1 \pts{\ndmnd} + \frac{1}{C_2}\pts{\ndpnd}}}{+C_3 \sqrt{n\nd}\nut+C_3 \sqrt{n\nd}\nuo}}^2}{C_4\nd d}\nonumber\\
         &\leq \frac{C \pts{\alpha_+R_+^2n_+ + \alpha_-R_-^2n_-}}{d},
    \end{align*}
    where we follow the same proof steps in Theorem~\ref{thm:wst_risk_upperbound}.
\end{proof}
\begin{proposition}\label{pro:ridge_wst_lower_bound}
Under Assumption~\ref{asm:dataset_gen}, the generalization error of ridge estimator for each group $b \in \{+1,-1\}$ is lower bounded as
    \begin{gather}
        \Riskf[b]{\hw}\geq C_1 \expf{- C_2 \frac{ \pts{\alpha_+R_b^2n_+ + \alpha_-R_{-b}^2n_-}}{d}},
    \end{gather}
    where $\alpha_\pm \coloneqq \frac{n_\pm/\Delta_\pm^2}{\nddpndd}=\frac{n_\pm/\Delta_\pm^2}{\nd}$ and $0 < \alpha_\pm < 1$.
\end{proposition}

\begin{proof}
    \begin{align}
        \frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} &= \frac{\pts{\y^\top\bDelta^{-1}\XXtaui\X\bmu_{+1}}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\nonumber\\
        &= \frac{\pts{\nut^2\stdtt + \nuo^2\stdot + \httdt + \hotdt}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\label{eq:ridge_maj_target_term},
    \end{align}
    where we reuse the primitives in Eq.~\eqref{eq:maj_target_primitive}. Next, we focus on lower bound the denominator.
    \begin{align*}
        &\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y\\
        &\geq \lambda_{\text{min}}\pts{\XXtaui\XX\XXtaui}\nnorm[2]{\bDelta^{-1}\y}^2\\
        &= \frac{\nnorm[2]{\bDelta^{-1}\y}^2}{\lambda_{\text{max}}\pts{\pts{\XXtau}\XXi\pts{\XXtau}}}\\
        &\geq \frac{\nnorm[2]{\bDelta^{-1}\y}^2}{\lambda_{\text{max}}\pts{\pts{\XXtau}}^2\lambda_{\text{max}}\pts{\XXi}}\\
        &= \frac{\lambda_{\text{min}}\pts{\XX}\nnorm[2]{\bDelta^{-1}\y}^2}{\pts{\lambda_{\text{max}}\pts{\XX}+\tau}^2}\\
        &\geq \frac{\frac{1}{C_1} d \nd}{C_2\pts{d+\tau}^2} = \frac{ d\nd}{C_3\pts{d+\tau}^2}.\\
    \end{align*}
    % where $a\coloneqq \lambda_{\text{min}}\pts{\XXtaui\XX\XXtaui}$.
    % And we have
    % \begin{align*}
    %     a &= \lambda_{\text{min}}\pts{\XXtaui\XX\XXtaui}\\
    %     &\geq \lambda_{\text{min}}\pts{\XXtaui}^2\lambda_{\text{min}}\pts{\XX}\\
    %     &= \frac{\lambda_{\text{min}}\pts{\XX}}{\lambda_{\text{max}}\pts{\XXtau}^2} = \frac{\lambda_{\text{min}}\pts{\XX}}{\pts{\lambda_{\text{max}}\pts{\XX} + \tau}^2}.
    % \end{align*}
    % Now, we need to find an upper bound for $\lambda_{\text{max}}\pts{\XX}$ and a lower bound for $\lambda_{\text{min}}\pts{\XX}$. By the definition of $\XX$, we have 
    % \begin{align*}
    %     \lambda_{\text{max}}\pts{\XX} &\leq \splitdfrac{\lambda_{\text{max}}\pts{\QQ} + \lambda_{\text{max}}\pts{\nuo^2\bv_1\bv_1^\top} + \lambda_{\text{max}}\pts{\bd_1\bv_1^\top + \bv_1\bd_1^\top}}{ + 
    %     \lambda_{\text{max}}\pts{\nut^2\bv_2\bv_2^\top} + 
    %     \lambda_{\text{max}}\pts{\bd_2\bv_2^\top + \bv_2\bd_2^\top}}\\
    %     &\leq C_1d + \nuo^2n + \nut^2 n + C_2n\nuo + C_3n\nut\\
    %     &\leq C_4 d,
    % \end{align*}
    % where we apply $d\geq CR_+n$.
    % \begin{align*}
    %     \lambda_{\text{min}}\pts{\XX} &\geq \splitdfrac{\lambda_{\text{min}}\pts{\QQ} + \lambda_{\text{min}}\pts{\nuo^2\bv_1\bv_1^\top} + \lambda_{\text{min}}\pts{\bd_1\bv_1^\top + \bv_1\bd_1^\top}}{ + 
    %     \lambda_{\text{min}}\pts{\nut^2\bv_2\bv_2^\top} + 
    %     \lambda_{\text{min}}\pts{\bd_2\bv_2^\top + \bv_2\bd_2^\top}}\\
    %     &\geq \frac{d}{C_5}.
    % \end{align*}
    % As a result, we get
    % \begin{align*}
    %     a \geq \frac{d}{C\pts{d + \tau}^2}.
    % \end{align*}
    % On the other hand, we have
    % \begin{align*}
    %     \text{Tr}\pts{\bDelta^{-1}\y\y^\top\bDelta^{-1}} = \text{Tr}\pts{\y^\top\bDelta^{-2}\y} = \nddpndd = \nd.
    % \end{align*}
    % Hence, we have 
    % \begin{align*}
    %     \y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y \geq \frac{\nd d}{C\pts{d+\tau}^2}.
    % \end{align*}
    Plug this in Eq.~\eqref{eq:ridge_maj_target_term}, we have
    \begin{align*}
         \frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} &= \frac{\pts{\nut^2\stdtt + \nuo^2\stdot + \httdt + \hotdt}^2}{2\y^\top\bDelta^{-1}\XXtaui\XX\XXtaui\bDelta^{-1}\y}\\
         &\leq \dfrac{\pts{\nut^2 \frac{\pts{\hc_1+\frac{1}{C_2}} \pts{\ndpnd}}{d+\tau} + \nuo^2 \frac{\hc_1 \pts{\ndmnd} + \frac{1}{C_2}\pts{\ndpnd}}{d+\tau}+\frac{C_3 \sqrt{n\nd}\nut}{d+\tau}+\frac{C_3 \sqrt{n\nd}\nuo}{d+\tau}}^2}{\frac{\nd d}{C_4\pts{d+\tau}^2}}\nonumber\\
         &\leq C_4\dfrac{\pts{\splitdfrac{\nut^2 \pts{\hc_1+\frac{1}{C_2}} \pts{\ndpnd} + \nuo^2 \pts{\hc_1 \pts{\ndmnd} + \frac{1}{C_2}\pts{\ndpnd}}}{+C_3 \sqrt{n\nd}\nut+C_3 \sqrt{n\nd}\nuo}}^2}{\nd d}\nonumber\\
         &\leq \frac{C \pts{\alpha_+R_+^2n_+ + \alpha_-R_-^2n_-}}{d},
    \end{align*}
    where we follow the same proof steps in Proposition~\ref{pro:wst_lower_bound}.
\end{proof}


==> proofs-explicit-primitives.tex <==
% \section{Proofs of primitive explicit result} \label{app:explicit_primitive_proof}


% \paragraph{bounds for $i=0$}
%     \begin{itemize}
%         \item $\saaz$:
%             \begin{align*}
%                 \saaz = \ba^\top\XXzi\ba = \ba^\top\QQi\ba.
%             \end{align*}
%             Follow the proof in~\cite{wang2022binary}, we have 
%             \begin{align*}
%                 \saaz &= \ba^\top\QQi\ba \leq \na^2\lbf[1]{\QQi}\leq\frac{n}{\lbf[n]{\QQ}}\leq \frac{Cn}{d},\\
%                 \saaz &= \ba^\top\QQi\ba \geq \na^2\lbf[n]{\QQi}\leq\frac{n}{\lbf[1]{\QQ}}\leq \frac{n}{Cd}.
%             \end{align*}
%         \item $\syyz$: The bounds for $\syyz$ are the same as $\saaz$.
%         \item $\syaz$: 
%             \begin{align*}
%                 \syaz = \y^\top\XXzi\ba = \y^\top\QQi\ba.
%             \end{align*}
%             Follow the proof in~\cite{wang2021benign}, we can use parallelogram law and have 
%             \begin{align*}
%                 \syaz = \y^\top\QQi\ba=\frac{1}{4}\pts{\pts{\y+\ba}^\top\QQi\pts{\y+\ba}-\pts{\y-\ba}^\top\QQi\pts{\y-\ba}}.
%             \end{align*}
%             Hence, we have 
%             \begin{align*}
%                 \syaz &\leq\frac{1}{4}\pts{4n_+\lbf[1]{\QQi} - 4n_-\lbf[n]{\QQi}}\leq\frac{Cn_+}{d}-\frac{n_-}{Cd},\\
%                 \syaz &\geq\frac{1}{4}\pts{4n_+\lbf[n]{\QQi} - 4n_-\lbf[1]{\QQi}}\geq\frac{n_+}{Cd}-\frac{Cn_-}{d}=-\pts{\frac{Cn_-}{d}-\frac{n_+}{Cd}}.
%             \end{align*}
%         \item $\tssz$: \kw{no lowerbound? revisit}
%             \begin{align*}
%                 \tssz = \bd_s^\top\XXzi\bd_s = \bd_s^\top\QQi\bd_s.
%             \end{align*}
%             Since we have $\nds\leq C\sqrt{n}\nus$, 
%             \begin{align*}
%                 \tssz &= \bd_s^\top\QQi\bd_s \leq Cn\nus^2\lbf[1]{\QQi}\leq\frac{Cn\nus^2}{\lbf[n]{\QQ}}\leq \frac{Cn\nus^2}{d}.
%             \end{align*}
%         \item $\tccz$: Similar to $\tssz$.
%         \item $\hsaz$:
%             \begin{align*}
%                 \hsaz = \bd_s^\top\XXzi\ba = \bd_s^\top\QQi\ba.
%             \end{align*}
%             Hence,
%             \begin{align*}
%                 \hsaz &\leq \nds\na\nnorm[2]{\QQi} \leq Cn\nus\lbf[1]{\QQi}\leq\frac{Cn\nus}{d},\\
%                 \hsaz &\geq -\nds\na\nnorm[2]{\QQi}\geq-\frac{Cn\nus}{d}.
%             \end{align*}
%         \item $\hsyz$, $\hcaz$ and $\hcyz$: Similar to $\hsaz$.
%     \end{itemize}

%     \paragraph{bounds for $i=1$}
%     \begin{itemize}
%         \item $\saao$:
%             \begin{align*}
%                 \saao = \ba^\top\XXoi\ba &= \ba^\top\XXzi\ba-\ba^\top\XXzi\bL_0\A_0^{-1}\bR_0\XXoi\ba,\\
%                 &=\saaz - \mts{\nus\saaz,~\hsaz,~\saaz}\frac{\text{adj}(\A_0)}{\det(\A_0)}\begin{bmatrix}
%                 \nus\saaz \\
%                 \saaz \\
%                 \hsaz
%                 \end{bmatrix}\\
%                 &=\saaz-\frac{1}{\det(\A_0)}\pts{\pts{\nus^2-\tssz}{\saaz}^2+{\hsaz}^2\saaz+2\hsaz\saaz}.
%             \end{align*}
%             To lowerbound $\saao$, we first upperbound $\frac{\pts{\nus^2-\tssz}{\saaz}^2}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\pts{\nus^2-\tssz}{\saaz}^2}{\det(\A_0)} \leq \frac{\pts{\nus^2-\tssz}{\saaz}^2}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\pts{\nus^2-\tssz}{\saaz}^2}{\saaz\pts{\nus^2-\tssz}}=\saaz
%             \end{align*}
%             Next, it's suffice to upperbound the dominant term $\frac{\hsaz\saaz}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\hsaz\saaz}{\det(\A_0)} \leq \frac{\hsaz\saaz}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\hsaz\saaz}{\pts{\hsaz+1}^2} \leq \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2}.
%             \end{align*}
%             Therefore, 
%             \begin{align*}
%                 \saao \geq \saaz - \saaz - \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2} \geq \frac{n}{Cd}.
%             \end{align*}
%             Similarly, we have upperbound such that
%             \begin{align*}
%                 \saao &\leq \normo{\saaz} + \frac{1}{\det(\A_0)}\normo{\pts{\nus^2-\tssz}{\saaz}^2+{\hsaz}^2\saaz+2\hsaz\saaz}\\
%                 &\leq \frac{Cn}{d} + \frac{Cn}{d} + \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2} \leq \frac{Cn}{d}.
%             \end{align*}
%         \item $\syyo$:
%             \begin{align*}
%                 \syyo = \y^\top\XXoi\y &= \y^\top\XXzi\y-\y^\top\XXzi\bL_0\A_0^{-1}\bR_0\XXoi\y,\\
%                 &=\syyz - \mts{\nus\syaz,~\hsyz,~\syaz}\frac{\text{adj}(\A_0)}{\det(\A_0)}\begin{bmatrix}
%                 \nus\syaz \\
%                 \syaz \\
%                 \hsyz
%                 \end{bmatrix}\\
%                 &=\syyz-\frac{1}{\det(\A_0)}\pts{\pts{\nus^2-\tssz}{\syaz}^2+ 2\hsaz\hsyz\syaz - {\hsyz}^2\saaz +2\hsyz\syaz}.
%             \end{align*}
%             To lowerbound $\syyo$, we first upperbound $\frac{\pts{\nus^2-\tssz}{\syaz}^2}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\pts{\nus^2-\tssz}{\syaz}^2}{\det(\A_0)} \leq \frac{\pts{\nus^2-\tssz}{\syaz}^2}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\pts{\nus^2-\tssz}{\syaz}^2}{\saaz\pts{\nus^2-\tssz}} \leq \frac{\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}^2}{\frac{n}{Cd}}
%             \end{align*}
%             Next, it's suffice to upperbound the dominant term $\frac{\hsyz\syaz}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\hsyz\syaz}{\det(\A_0)} \leq \frac{\hsyz\syaz}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\hsyz\syaz}{\pts{\hsaz+1}^2} \leq \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2}.
%             \end{align*}
%             Therefore, 
%             \begin{align*}
%                 \syyo \geq \syyz - \frac{\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}^2}{\frac{n}{Cd}} - \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2} \geq \frac{n}{Cd}.
%             \end{align*}
%             Similarly, we have upperbound such that
%             \begin{align*}
%                 \syyo &\leq \normo{\syyz} + \frac{1}{\det(\A_0)}\normo{\pts{\nus^2-\tssz}{\syaz}^2+ 2\hsaz\hsyz\syaz - {\hsyz}^2\saaz +2\hsyz\syaz}\\
%                 &\leq \frac{Cn}{d} + \frac{\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}^2}{\frac{n}{Cd}} + \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2} \leq \frac{Cn}{d}.
%             \end{align*}
%         \item $\syao$:
%             \begin{align*}
%                 \syao = \y^\top\XXoi\ba &= \y^\top\XXzi\ba-\y^\top\XXzi\bL_0\A_0^{-1}\bR_0\XXoi\ba,\\
%                 &=\syaz - \mts{\nus\syaz,~\hsyz,~\syaz}\frac{\text{adj}(\A_0)}{\det(\A_0)}\begin{bmatrix}
%                 \nus\saaz \\
%                 \saaz \\
%                 \hsaz
%                 \end{bmatrix}\\
%                 &=\syaz-\frac{1}{\det(\A_0)}\pts{\pts{\nus^2-\tssz}\syaz\saaz + {\hsaz}^2\syaz + \hsaz\syaz +\hsyz\saaz}.
%             \end{align*}
%             To lowerbound $\syao$, we first upperbound $\frac{\pts{\nus^2-\tssz}\syaz\saaz}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\pts{\nus^2-\tssz}\syaz\saaz}{\det(\A_0)} \leq \frac{\pts{\nus^2-\tssz}\syaz\saaz}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\pts{\nus^2-\tssz}\syaz\saaz}{\saaz\pts{\nus^2-\tssz}} \leq \frac{C n_+}{d} - \frac{n_-}{C d}.
%             \end{align*}
%             Next, it's suffice to upperbound the dominant term $\frac{\hsaz\syaz}{\det(\A_0)}$ and $\frac{\hsyz\saaz}{\det(\A_0)}$.
%             \begin{align*}
%                 \frac{\hsaz\syaz}{\det(\A_0)} \leq \frac{\hsaz\syaz}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\hsaz\syaz}{\pts{\hsaz+1}^2} \leq \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2}.
%             \end{align*}
%             \begin{align*}
%                 \frac{\hsyz\saaz}{\det(\A_0)} \leq \frac{\hsyz\saaz}{\saaz\pts{\nus^2-\tssz}+\pts{\hsaz+1}^2} \leq \frac{\hsyz\saaz}{\pts{\hsaz+1}^2} \leq \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2}.
%             \end{align*}
%             Therefore, 
%             \begin{align*}
%                 \syao \geq \syaz - \pts{\frac{C n_+}{d} - \frac{n_-}{C d}} - \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2} - \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2} \geq \frac{n_+}{C d} - \frac{C n_-}{d}.
%             \end{align*}
%             Similarly, we have upperbound such that
%             \begin{align*}
%                 \syao &\leq \normo{\syaz} + \frac{1}{\det(\A_0)}\normo{\pts{\nus^2-\tssz}\syaz\saaz + {\hsaz}^2\syaz + \hsaz\syaz +\hsyz\saaz}\\
%                 &\leq \pts{\frac{C n_+}{d} - \frac{n_-}{C d}} + \pts{\frac{C n_+}{d} - \frac{n_-}{C d}} + \frac{\frac{Cn\nus}{d}\pts{\frac{C n_+}{d} - \frac{n_-}{C d}}}{\pts{1-\frac{Cn\nus}{d}}^2} + \frac{\frac{Cn\nus}{d}\frac{Cn}{d}}{\pts{1-\frac{Cn\nus}{d}}^2} \leq \frac{C n_+}{d} - \frac{n_-}{C d}.
%             \end{align*}
%     \end{itemize}

==> proofs-upperbound.tex <==
\section{Proof of Theorem~\ref{thm:wst_risk_upperbound}} \label{app:upperbound_proof}
In this section, we present the proof of Theorem~\ref{thm:wst_risk_upperbound} in four steps. We first present the upper bound of the worst group classification risk in analytical form for majority and minority group. Next, in order to simplify the calculation of the analytical upper bound, we define "primitive" quadratic terms and derive their upper and lower bounds respectively in step 2 \& 3. Finally, we substitute all terms in the classification risk upper bound with primitives and apply their bounds to achieve the upper bound result of Theorem~\ref{thm:wst_risk_upperbound} for both groups.\\
%
\textbf{Step 1.} Recall the upper bound of worst group classification risk in Lemma~\ref{lem:wst_risk_q_upper} such as
%
\begin{align}\label{eq:wst_risk_q_upper}
    \Riskf[wst]{\hw} \leq \umax{b\in\pm1}~\expf{-\frac{\pts{\hw^\top\bmu_b}^2}{2\hw^{\top}\hw}}.
\end{align}
%
Eq.~\eqref{eq:wst_risk_q_upper} basically shows that the worst group classification risk is upper bound by the exponential term either from majority ($b=+1$) or minority ($b=-1$) group, and such term involves the product of $\hw$ and mean vector of group $b$ and the quadratic term of $\hw$. Therefore, our goal is to understand the relationship between $\hw$ and mean vector and to derive an lower bound of $\frac{\pts{\hw^\top\bmu_b}^2}{2\hw^{\top}\hw}$ for each $b\in\pm1$. Next, we substitute $\hw$ in Eq.~\eqref{eq:wst_risk_q_upper} with the closed form interpolation of cMNI Eq.~\eqref{eq:sq_sol} to get
%
\begin{align}\label{eq:target_term_repeat}
    \frac{\pts{\hw^\top\bmu_b}^2}{2\hw^{\top}\hw}
    &=\frac{\pts{\y^\top\bDelta^{-1}\XXi\X\bmu_b}^2}{2\y^\top\bDelta^{-1}\XXi\bDelta^{-1}\y}.
\end{align}
%
As a result, we can achieve an analytical lower bound of Eq.~\eqref{eq:target_term_repeat} by analyzing the properties and dynamics between dataset matrix $\X$, $\y$, adjustment weight $\bDelta$ and mean vector $\bmu_b$ in each group in the following steps.\\
%
\textbf{Step 2.} In order to analyze and upper bound Eq.~\eqref{eq:target_term_repeat}, we start with showing notations and calculations which help analyze the Gram matrix $\XX$ and its inverse. According to the definition of $\X$ in Eq.~\eqref{eq:x_matrix_def}, we have
%
\begin{align*}
    \XX &= (\y\barmu_c^\top+\ba\barmu_s^\top+\Q)(\y\barmu_c^\top+\ba\barmu_s^\top+\Q)^\top\nonumber\\
    &\coloneqq (\bv_2\barmu_2^\top+\bv_1\barmu_1^\top+\Q)(\bv_2\barmu_2^\top+\bv_1\barmu_1^\top+\Q)^\top,
\end{align*}
%
where we denote $\bv_1 \coloneqq \ba$, $\bv_2 \coloneqq \y$, $\barmu_1 \coloneqq \barmu_s$, $\barmu_1 \coloneqq \barmu_c$ for ease of later recursive calculations. Note that since there are correct and spurious mean vectors going along with the Wishart matrix $\QQ$ inside $\XX$, it's not easy to directly analyze and show inequalities for $\XX$ and it inverse. To overcome this challenge, followed by the idea in~\cite{wang2021benign}, we can decompose the data matrix $\X$ in orders such that
%
\begin{gather}
    \X_0 \coloneqq \Q, \quad \X_1 \coloneqq \bv_1\barmu_1^\top + \X_0, \quad \X_2 \coloneqq \bv_2\barmu_2^\top + \X_1,\nonumber
    % \X_0&:=\Q, \quad \\
    % \X_1&:=\bv_1\barmu_1^\top + \X_0 = \ba\barmu_s^\top + \Q\\
    % \X=\X_2&:=\bv_2\barmu_2^\top + \X_1 = \y\barmu_c^\top + \ba\barmu_s^\top + \Q,
\end{gather}
and for $k=1,2$,
\begin{align}
    \XXz &= \QQ\nonumber\\
    \XXk &= \pts{\bv_k\barmu_k^\top+\X_{k-1}}\pts{\bv_k\barmu_k^\top+\X_{k-1}}^\top\nonumber\\
         &= \XXkmo+\underbrace{\mts{\nuo\bv_k,~\bd_k,~\bv_k}}_{=:\bL_k}\underbrace{\begin{bmatrix}
         \nuo\bv_k^\top \\
         \bv_k^\top \\
         \bd_k^\top
         \end{bmatrix}}_{=:\bR_k},\label{eq:xx_def}
\end{align}
%
% \begin{align}
%     \XXz &= \QQ\\
%     \XXo &= \pts{\bv_1\barmu_1^\top+\X_0}\pts{\bv_1\barmu_1^\top+\X_0}^\top\nonumber\\
%          &= \XXz+\underbrace{\mts{\nuo\bv_1,~\bd_1,~\bv_1}}_{=:\bL_1}\underbrace{\begin{bmatrix}
%          \nuo\bv_1^\top \\
%          \bv_1^\top \\
%          \bd_1^\top
%          \end{bmatrix}}_{=:\bR_1}\\
%     \XXt &= \pts{\bv_2\barmu_2^\top+\X_1}\pts{\bv_2\barmu_c^\top+\X_1}^\top\nonumber\\
%          &= \XXo+\underbrace{\mts{\nut\bv_2,~\bd_2,~\bv_2}}_{=:\bL_2}\underbrace{\begin{bmatrix}
%          \nut\bv_2^\top \\
%          \bv_2^\top \\
%          \bd_2^\top
%          \end{bmatrix}}_{=:\bR_2},
% \end{align}
%
where we denote $\bL_k$, $\bR_k$ matrix respectively, and $\bd_k:=\X_{k-1}\barmu_k=\Q\barmu_k$, since $\barmu_1$ and $\barmu_2$ are orthogonal to each other. Next, resembled to the $\XXi$ derivation in~\cite{wang2021benign}, we apply recursive Woodbury identity~\cite{horn2012matrix} to break the matrix inversion calculation into recursive steps such that
%
\begin{align}
    &\XXzi = \QQi\nonumber\\
    &\XXki = \XXkmoi \nonumber\\
           &- \XXkmoi \bL_{k}\A_k^{-1}\bR_k\XXkmoi,\label{eq:xxi_def}
    % \pts{\underbrace{\I+\bR_k\XXkmoi\bL_k}_{=:\A_k}}^{-1}
\end{align}
%
where $\A_k \coloneqq \I+\bR_k\XXkmoi\bL_k$ for $k=1,2$. As a result, we can represent the $k$th order inverse Gram matrix $\XXki$ into multiplication of previous order inverse Gram matrix $\XXkmoi$. By applying the operation recursively, we can derive $\XXi$ which is in the $2$nd order into multiplication of matrices in $0$th order which is $\QQi$.\\
%
\textbf{Step 3.} Equipped with the tools derived in Step 2, we are ready to analyze the lower bound of Eq.~\eqref{eq:target_term_repeat}. Inspired by~\cite{wang2022binary,wang2021benign}, we define several "primitive" quadratic terms involving $\XXki$ in each order in order to decompose the derivation of inequalities into parts in the following definition.
%
\begin{definition}\label{def:primitives}
    We define the following primitive quadratic terms.
    \begin{gather}
        \sijk \coloneqq \bv_i^\top\XXki\bv_j,\quad \tijk \coloneqq \bd_i^\top\XXki\bd_j,\nonumber\\
        \hijk \coloneqq \bd_i^\top\XXki\bv_j \nonumber,\nonumber
    \end{gather}
    for $i, j = 1, 2$ and order $k=0,1,2$.
\end{definition}
%
Note that additional to basic primitives in Def.~\ref{def:primitives}, we also define primitives with adjustment weight in setup since Eq.~\eqref{eq:target_term_repeat} possesses adjustment weight matrix $\bDelta$. Thus, we have the following definition.
%
\begin{definition}\label{def:w_primitives}
    We define the following primitive quadratic terms with adjustment weight.
    \begin{gather}
        \sidjk \coloneqq \bv_i^\top\bDelta^{-1}\XXki\bv_j,\nonumber\\
        \sidjdk \coloneqq \bv_i^\top\bDelta^{-1}\XXki\bDelta^{-1}\bv_j,\nonumber\\
        \hijdk\coloneqq \bd_i^\top\XXki\bDelta^{-1}\bv_j,\nonumber
    \end{gather}
    for $i, j = 1, 2$ and order $k=0,1,2$.
\end{definition}
%
Next, since these primitives involving $\XXki$ in each order can be converted into multiplication of matrices with $\QQi$, we can apply concentration inequalities on inverse Wishart matrix $\QQi$ and derive upper and lower bounds for all primitives. We present the bounds of primitives in the following lemmas. We categorize these primitive bounds in square terms ($i=j$) or cross terms ($i \neq j$). Additionally, we also need bounds for product of determinant of $\A_k$ in each order to achieve the lower bound of Eq.\eqref{eq:target_term_repeat}. Full proofs for Lemma~\ref{lem:primitive_bounds} and Lemma~\ref{lem:w_primitive_bounds} are in Appendix~\ref{app:primitive_proof}.
%
\begin{lemma}\label{lem:primitive_bounds}
    For primitives we defined in Def.~\ref{def:primitives}, for some $C_1,C_2,C_3,C_4,C_5>1$ and $\hc_m \coloneqq \frac{C_m+1}{C_m}$ and $\dc_m \coloneqq \frac{C_m-1}{C_m}$, we have the following bounds.
    \begin{gather*}
        \dc_1\frac{n}{d}\leq \siik \leq \hc_{1}\frac{n}{d}\\
        \dc_2\frac{n_+}{d} - \hc_2\frac{n_-}{d} \leq \sotk \leq \hc_2\frac{n_+}{d} - \dc_2\frac{n_-}{d}\\
        \tiik \leq \frac{C_3 n\nui^2}{d}\\
        -\frac{C_4 n\nuo\nut}{d}\leq \totk \leq \frac{C_4 n\nuo\nut}{d}\\
        -\frac{C_5 n\nui}{d}\leq \hijk \leq \frac{C_5 n\nui}{d}
    \end{gather*}
    for $i, j = 1, 2$ and order $k=0,1,2$.
\end{lemma}
%
\begin{lemma}\label{lem:w_primitive_bounds}
    For primitives we defined in Def.~\ref{def:w_primitives}, for some $C_1,C_2,C_3,C_4>1$, and $\hc_m \coloneqq \frac{C_m+1}{C_m}$ and $\dc_m \coloneqq \frac{C_m-1}{C_m}$, we have the following bounds.
    \begin{gather*}
        \frac{\pts{\hc_1-\frac{1}{C_2}}\pts{\ndpnd}}{d}\leq \sidik \leq \frac{\pts{\hc_1+\frac{1}{C_2}}\pts{\ndpnd}}{d}\\
        %
        \frac{\splitfrac{\hc_1 \pts{\ndmnd}}{- \frac{1}{C_2}\pts{\ndpnd}}}{d}\leq \stdok \leq \frac{\splitfrac{\hc_1 \pts{\ndmnd}}{+ \frac{1}{C_2}\pts{\ndpnd}}}{d}\\
        %
        \frac{\dc_3\nd}{d}\leq \sididk \leq \frac{\hc_3 \nd}{d}\\
        %
        -\frac{C_4 \sqrt{n\nd}\nui}{d}\leq \hijdk \leq \frac{C_4 \sqrt{n\nd}\nui}{d},
    \end{gather*}
    % where $D_0=1$, $D_k:=D_{k-1}\det(\A_k)$ 
    where $\nd \coloneqq \frac{n_+}{\Delta_+^2}+\frac{n_-}{\Delta_-^2}$ for $i, j = 1, 2$ and order $k=0,1,2$.
\end{lemma}
%
Note that primitives defined in Def.~\ref{def:primitives} and their bounds in Lemma~\ref{lem:primitive_bounds} won't be used directly in the proof of Theorem\ref{thm:wst_risk_upperbound}, but they will be used in recursive Woodbury identity calculation.
%
% \begin{lemma}\label{lem:det_bound}
%     We define $D_0=1$ and $D_k:=D_{k-1}\det(\A_k)$. For some $C_1,C_2>1$, we have\kw{complete the lower bound here}
%     \begin{align*} 
%         C_1 - \frac{C_2 n}{d}R_+ \leq D_k \leq C_1 + \frac{C_2 n}{d}R_+.
%     \end{align*}
% \end{lemma}
%
\textbf{Step 4.} With the primitives with adjustment weight derived in Def~\ref{def:w_primitives}, we can substitute terms in Eq.~\eqref{eq:target_term_repeat} with those primitives. We demonstrate the derivation of majority group case only since the minority group case follows by the same calculations.
%
\begin{align}
    &\frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} = \frac{\pts{\y^\top\Delta^{-1}\XXi\X\bmu_{+1}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\nonumber\\
    &= \frac{\pts{\y^\top\Delta^{-1}\XXi\pts{\y\barmu_c^\top + \ba\barmu_s^\top+\Q}\pts{\barmu_c + \barmu_s}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\nonumber\\
    &= \frac{\pts{\bv_2^\top\Delta^{-1}\XXti\pts{\bv_2\barmu_2^\top + \bv_1\barmu_1^\top+\Q}\pts{\barmu_2 + \barmu_1}}^2}{2\bv_2^\top\Delta^{-1}\XXti\Delta^{-1}\bv_2}\nonumber\\
    &= \frac{\pts{\nut^2\stdtt + \nuo^2\stdot + \httdt + \hotdt}^2}{2\stdtdt}\label{eq:maj_target_primitive},
\end{align}
where the second equality follows by the definition of $\bmu_{+1}=\barmu_c + \barmu_s$ and the definition of $\X$, and we apply the recursive notation in third equality and substitute all terms with primitives in Def.~\ref{def:w_primitives} in the last equality. Right before we put together primitive bounds, we need the following auxiliary lemma to help us simplify terms. We defer proof of Lemma~\ref{lem:aux_compare_a_h} in Appendix~\ref{app:aux_lem_proof}.
%
\begin{lemma}\label{lem:aux_compare_a_h}
    For some $C>C_1>0$, if $\nut^2 \geq Cn\log(n/\delta)$ or $n_-$ is a factor of $n$ such that $n_-=\alpha n$ for $0 < \alpha \leq 1/2$, we have
    \begin{align*}
        \frac{1}{2}\pts{\ndpnd}\nut &\geq C_1\sqrt{n\nd}.
    \end{align*}
\end{lemma}
%
Finally, we can introduce the primitive bounds in Lemma~\ref{lem:w_primitive_bounds} into Eq.~\eqref{eq:maj_target_primitive}. In order to get a lower bound of Eq.~\eqref{eq:maj_target_primitive}, we will lower bound the numerator and upper bound the denominator. Thus, we get
%
\begin{align}
    \eqref{eq:maj_target_primitive}&\geq \dfrac{\pts{\splitdfrac{\nut^2 \frac{\pts{\hc_1-\frac{1}{C_2}} \pts{\ndpnd}}{d}}{\splitdfrac{ + \nuo^2 \frac{\hc_1 \pts{\ndmnd} - \frac{1}{C_2}\pts{\ndpnd}}{d}}{-\frac{C_3 \sqrt{n\nd}\nuc}{d}-\frac{C_3 \sqrt{n\nd}\nus}{d}}}}^2}{\frac{\hc_4 \nd}{ d}}\nonumber\\
    &= \dfrac{\pts{\splitdfrac{\pts{\hc_1\nut^2 -\frac{\nut^2+\nuo^2}{C_2}}\pts{\ndpnd}}{\splitdfrac{+ \hc_1 \nuo^2\pts{\ndmnd}}{-C_3 \sqrt{n\nd}\pts{\nut+\nuo}}}}^2}{\hc_4 \nd d}.\label{eq:maj_target_primitive_1}
\end{align}
Next, since we assume $R_- \geq 0$ or $\nut \geq \nuo$, we get
\begin{align}
    \eqref{eq:maj_target_primitive_1} &\geq \dfrac{\pts{\splitdfrac{\pts{\hc_1\nut^2 -\frac{2\nut^2}{C_2}}\pts{\ndpnd}}{\splitdfrac{+ \hc_1 \nuo^2\pts{\ndmnd}}{-2C_3 \sqrt{n\nd}\nut}}}^2}{\hc_4 \nd d}\nonumber\\
    &\geq \dfrac{\pts{\splitdfrac{\pts{\hc_1 -\frac{2}{C_2} -\frac{C_3}{C_5}}\nut^2\pts{\ndpnd}}{+ \hc_1 \nuo^2\pts{\ndmnd}}}^2}{\hc_4 \nd d}\nonumber\\
    &= \dfrac{\pts{\hc_6\nut^2\pts{\ndpnd} + \hc_6 \nuo^2\pts{\ndmnd}}^2}{\hc_4 \nd d}\nonumber\\
    &= \dfrac{\pts{\hc_6 R_+\frac{n_+}{\Delta_+} + \hc_6 R_-\frac{n_-}{\Delta_-}}^2}{\hc_4 \nd d} \geq \dfrac{\hc_6^2 R_+^2\frac{n_+^2}{\Delta_+^2} + \hc_6^2 R_-^2\frac{n_-^2}{\Delta_-^2}}{\hc_4\nd d},\label{eq:maj_target_primitive_2}
\end{align}
where the second inequality follows by Lemma~\ref{lem:aux_compare_a_h} with $C_5 > C_3$. In the last inequality, we subtract the cross term in numerator. Next, we define 
\begin{align*}
    \alpha_\pm = \frac{\frac{n_\pm}{\Delta_\pm^2}}{\nddpndd}=\frac{\frac{n_\pm}{\Delta_\pm^2}}{\nd},
\end{align*}
where $0<\alpha_\pm<1$ and $\alpha_+ + \alpha_-=1$. Then, Eq.~\eqref{eq:maj_target_primitive_2} becomes
\begin{align*}
    \frac{\pts{\hw^\top\bmu_{+1}}^2}{2\hw^{\top}\hw} &\geq \frac{\hc_6^2 \pts{\alpha_+R_+^2 n_+ + \alpha_-R_-^2 n_-}}{\hc_4 d}\\
    &= \frac{\hc_7 \pts{\alpha_+R_+^2\frac{n_+}{n} + \alpha_-R_-^2\frac{n_-}{n}}}{d/n}.
\end{align*}
%
% On the other hand, for minority group $b=-1$, followed by Eq.~\eqref{eq:target_term_repeat} and the same steps, we have
% %
% \begin{align}
%     &\frac{\pts{\hw^\top\bmu_{-1}}^2}{2\hw^{\top}\bSigma\hw} = \frac{\pts{\y^\top\Delta^{-1}\XXi\X\bmu_{-1}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\nonumber\\
%     &= \frac{\pts{\y^\top\Delta^{-1}\XXi\pts{\y\barmu_c^\top + \ba\barmu_s^\top+\Q}\pts{\barmu_c - \barmu_s}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\nonumber\\
%     &= \frac{\pts{\nuc^2\sydyt-\nus^2\sydat + \hcydt - \hsydt}^2}{2\sydydt}\label{eq:min_target_primitive}.
% \end{align}
% %
% Note that the only difference between majority Eq.\eqref{eq:maj_target_primitive} and minority Eq.\eqref{eq:min_target_primitive} is the signs are flipped in second and fourth terms in the numerator. Again, by introducing Lemma~\ref{lem:w_primitive_bounds}, we can get the lower bound result of minority group as 
% %
% \begin{align*}
%     &\frac{\pts{\hw^\top\bmu_{-1}}^2}{2\hw^{\top}\bSigma\hw}\\
%     &\geq \dfrac{\pts{\splitdfrac{\nuc^2 \frac{C_1 \pts{\ndpnd} - \frac{\Delta_-}{C_1}\pts{n + \nd}}{D_2d}}{\splitdfrac{ - \nus^2 \frac{C_1 \pts{\ndmnd} + \frac{\Delta_-}{C_1}\pts{n + \nd}}{D_2d}}{ -\frac{C_2 n\sqrt{\frac{\nd}{n}}\nuc}{D_2d}-\frac{C_2 n\sqrt{\frac{\nd}{n}}\nus}{D_2d}}}}^2}{\frac{C_3 \nd}{D_2d}}\\
%     &= \dfrac{\pts{\splitdfrac{C_1 R_-\frac{n_+}{\Delta_+} + C_1 R_+\frac{n_-}{\Delta_-} -\frac{\Delta_-}{C_1}R_+\pts{n + \nd}}{-C_2 \pts{\nuc +\nus} n\sqrt{\frac{\nd}{n}} }}^2}{C_3 D_2 d\nd}\\
%     &= \dfrac{\pts{\splitdfrac{C_1 R_-\frac{n_+}{n\Delta_+} + C_1 R_+\frac{n_-}{n\Delta_-} -\frac{\Delta_-}{C_1}R_+\pts{1 + \frac{\nd}{n}}}{-C_2 \pts{\nuc +\nus} \sqrt{\frac{\nd}{n}} }}^2}{C_3 D_2 d\frac{\nd}{n^2}}\\
%     &\geq \dfrac{\pts{\splitdfrac{C_1 R_-\frac{n_+}{n\Delta_+} + C_1 R_+\frac{n_-}{n\Delta_-} -\frac{\Delta_-}{C_1}R_+\pts{1 + \frac{\nd}{n}}}{-C_2 \pts{\nuc +\nus}\sqrt{\frac{\nd}{n}} }}^2}{C_3 \frac{\nd}{n}\pts{C_4 R_+ +C_5\frac{d}{n}}}\\
%     &= \dfrac{\pts{C_6 R_-\frac{n_+}{n\Delta_+} + C_7 R_+\frac{n_-}{n\Delta_-} }^2}{C_4 R_+ +C_5\frac{d}{n}}\\
%     &= \dfrac{\pts{C_6 R_-\frac{n_+}{n\Delta_+} + C_7 R_+\frac{n_-}{n\Delta_-} }^2}{C_8\frac{d}{n}}.
% \end{align*}
%
% \begin{proof} (of Theorem~\ref{thm:lowerbound})

% For group $b=+1$,
% \begin{align*}
%     \frac{\pts{\hw^\top\barmu_{+1}}^2}{2\hw^{\top}\Sigma\hw}&=\frac{\pts{\y^\top\Delta^{-1}\XXi\X\barmu_{+1}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\\
%     &=\frac{\pts{\y^\top\Delta^{-1}\XXi\pts{\y\barmu_c + \ba\barmu_s+\Q}\pts{\barmu_c + \barmu_s}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}
% \end{align*}
% For the numerator,
% \begin{align*}
%     \text{numerator}&=(\y^\top\Delta^{-1}\XXi\y\nnorm[2]{\barmu_c}^2+\y^\top\Delta^{-1}\XXi\ba\nnorm[2]{\barmu_s}^2\\ 
%     &+ \y^\top\Delta^{-1}\XXi\Q\barmu_c + \y^\top\Delta^{-1}\XXi\Q\barmu_s)^2\\
%     &=\pts{s_{yy\Delta}^{\pts{2}}\nnorm[2]{\barmu_c}^2 + s_{ya\Delta}^{\pts{2}}\nnorm[2]{\barmu_s}^2+h_{cy\Delta}^{\pts{2}}+h_{sy\Delta}^{\pts{2}}}^2.
% \end{align*}
% For the denominator
% \begin{align*}
%     \text{denominator}&=2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y=s_{yy\Delta\Delta}^{\pts{2}}.
% \end{align*}
% From Lemma~\ref{lem:primitive_bounds}, we have
% \begin{align*}
%     \frac{n}{C_1 d}\leq &s_{yy\Delta}^{\pts{2}} \leq \frac{C_1 n}{\Delta d}\\
%     -\frac{C_2 n}{\Delta d}\leq &s_{ya\Delta}^{\pts{2}} \leq \frac{C_2 n}{\Delta d}\\
%     -\frac{C_3 n\nnorm[2]{\barmu_c}}{\Delta d}\leq &h_{cy\Delta}^{\pts{2}} \leq \frac{C_3 n\nnorm[2]{\barmu_c}}{\Delta d}\\
%     -\frac{C_4 n\nnorm[2]{\barmu_s}}{\Delta d}\leq &h_{sy\Delta}^{\pts{2}} \leq \frac{C_4 n\nnorm[2]{\barmu_s}}{\Delta d}\\
%     \frac{n}{C_5 d}\leq &s_{yy\Delta\Delta}^{\pts{2}} \leq \frac{C_5 n}{\Delta^2 d}.\\
% \end{align*}
% By plugging in these primitive bounds, we have 
% \begin{align*}
%     \text{numerator} \geq \pts{\frac{n}{C_1 d}\nnorm[2]{\barmu_c}^2 -\frac{C_2 n}{\Delta d}\nnorm[2]{\barmu_s}^2-\frac{C_3 n\nnorm[2]{\barmu_c}}{\Delta d}-\frac{C_4 n\nnorm[2]{\barmu_s}}{\Delta d}}^2,
% \end{align*}
% and
% \begin{align*}
%     \text{denominator} \leq \frac{C_5 n}{\Delta^2 d}.
% \end{align*}
% As a result,
% \begin{align*}
% \frac{\pts{\hw^\top\barmu_{+1}}^2}{2\hw^{\top}\Sigma\hw} &\geq \frac{\pts{\frac{n}{C_1 d}\nnorm[2]{\barmu_c}^2 -\frac{C_2 n}{\Delta d}\nnorm[2]{\barmu_s}^2-\frac{C_3 n\nnorm[2]{\barmu_c}}{\Delta d}-\frac{C_4 n\nnorm[2]{\barmu_s}}{\Delta d}}^2}{\frac{C_5 n}{\Delta^2 d}}\\
% &=\frac{n\pts{\frac{\Delta}{C_1}\nnorm[2]{\barmu_c}^2 -C_2\nnorm[2]{\barmu_s}^2-C_3\nnorm[2]{\barmu_c}-C_4\nnorm[2]{\barmu_s}}^2}{C_5 d}.
% \end{align*}
% Similarly, for group $b=-1$,
% \begin{align*}
%     \frac{\pts{\hw^\top\barmu_{-1}}^2}{2\hw^{\top}\Sigma\hw}&=\frac{\pts{\y^\top\Delta^{-1}\XXi\X\barmu_{-1}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}\\
%     &=\frac{\pts{\y^\top\Delta^{-1}\XXi\pts{\y\barmu_c + \ba\barmu_s+\Q}\pts{\barmu_c - \barmu_s}}^2}{2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y}
% \end{align*}
% For the numerator,
% \begin{align*}
%     \text{numerator}&=(\y^\top\Delta^{-1}\XXi\y\nnorm[2]{\barmu_c}^2-\y^\top\Delta^{-1}\XXi\ba\nnorm[2]{\barmu_s}^2\\ 
%     &+ \y^\top\Delta^{-1}\XXi\Q\barmu_c - \y^\top\Delta^{-1}\XXi\Q\barmu_s)^2\\
%     &=\pts{s_{yy\Delta}^{\pts{2}}\nnorm[2]{\barmu_c}^2 - s_{ya\Delta}^{\pts{2}}\nnorm[2]{\barmu_s}^2+h_{cy\Delta}^{\pts{2}}-h_{sy\Delta}^{\pts{2}}}^2.
% \end{align*}
% For the denominator
% \begin{align*}
%     \text{denominator}&=2\y^\top\Delta^{-1}\XXi\Delta^{-1}\y=s_{yy\Delta\Delta}^{\pts{2}}.
% \end{align*}
% By plugging in primitive bounds, we get
% \begin{align*}
% \frac{\pts{\hw^\top\barmu_{-1}}^2}{2\hw^{\top}\Sigma\hw} &\geq \frac{\pts{\frac{n}{C_1 d}\nnorm[2]{\barmu_c}^2 -\frac{C_2 n}{\Delta d}\nnorm[2]{\barmu_s}^2-\frac{C_3 n\nnorm[2]{\barmu_c}}{\Delta d}-\frac{C_4 n\nnorm[2]{\barmu_s}}{\Delta d}}^2}{\frac{C_5 n}{\Delta^2 d}}\\
% &=\frac{n\pts{\frac{\Delta}{C_1}\nnorm[2]{\barmu_c}^2 -C_2\nnorm[2]{\barmu_s}^2-C_3\nnorm[2]{\barmu_c}-C_4\nnorm[2]{\barmu_s}}^2}{C_5 d}.
% \end{align*}

% \end{proof}
